Coding for the unsourced B-channel with erasures: enhancing the linked loop code

In [1], the linked loop code (LLC) is presented as a promising code for the unsourced A-channel with erasures (UACE). The UACE is an unsourced multiple access channel in which active users' transmitted symbols are erased with a given probability and the channel output is obtained as the union of the non-erased symbols. In this paper, we extend the UACE channel model to the unsourced B-channel with erasures (UBCE). The UBCE differs from the UACE in that the channel output is the multiset union, or bag union, of the non-erased input symbols. In other words, the UBCE preserves the symbol multiplicity of the channel output while the UACE does not. Both the UACE and UBCE find applications in modeling aspects of unsourced random access. The LLC from [1] is enhanced and shown to outperform the tree code over the UBCE. Findings are supported by numerical simulations.

==> Figures/llc_structure.tex <==
\begin{tikzpicture}
[font=\small, draw=black,  >=stealth', line width=0.75pt,
sub0/.style={rectangle, draw, inner sep=0pt, minimum width=10mm, minimum height=2.5mm},
parity/.style={rectangle, draw, fill=lightgray, inner sep=0pt, minimum size=2.5mm}]

\foreach \c in {0.00} {
  \node[sub0] (subcs1\c) at (-1.00,\c) {};
  \node[parity] (parity1a\c) at (-0.875,\c) {};
  \node[parity] (parity1b\c) at (-0.625,\c) {};
  \node[sub0] (subcs2\c) at (0.50,\c) {};
  \node[parity] (parity2a\c) at (0.625,\c) {};
  \node[parity] (parity2b\c) at (0.875,\c) {};
  \node[sub0] (subcs3\c) at (2.00,\c) {};
  \node[parity] (parity3a\c) at (2.125,\c) {};
  \node[parity] (parity3b\c) at (2.375,\c) {};
  \node[sub0] (subcs4\c) at (3.50,\c) {};
  \node[parity] (parity4a\c) at (3.625,\c) {};
  \node[parity] (parity4b\c) at (3.875,\c) {};
  \node[sub0] (subcs5\c) at (5.00,\c) {};
  \node[parity] (parity5a\c) at (5.125,\c) {};
  \node[parity] (parity5b\c) at (5.375,\c) {};
}

\draw [->] (-1.25,0.2) to [out=45,in=135] (0.75,0.2);
\draw [->] (-1.25,0.2) to [out=45,in=135] (2.25,0.2);
\draw [->,densely dashed] (0.25,0.2) to [out=45,in=135] (2.25,0.2);
\draw [->,densely dashed] (0.25,0.2) to [out=45,in=135] (3.75,0.2);
\draw [->, densely dotted] (1.75,0.2) to [out=45,in=135] (3.75,0.2);
\draw [->, densely dotted] (1.75,0.2) to [out=45,in=135] (5.25,0.2);
\draw [->, dotted] (3.25,0.2) to [out=45,in=135] (5.25,0.2);
\draw [-, dotted] (3.25,0.2) to [out=45,in=180] (5.25,1);
\draw [->, loosely dotted] (-1.50,1) to [out=0,in=135] (0.75,0.2);

\node (info0) at (-1,-0.5) {$\wv(0)\pv(0)$};
% \node (par0) at (-0.75,-0.5) {$$};
\node (info1) at (0.5,-0.5) {$\wv(1)\pv(1)$};
% \node (par1) at (0.75,-0.5) {$$};
\node (info2) at (2,-0.5) {$\wv(2)\pv(2)$};
% \node (par2) at (2.25,-0.5) {$$};
\node (info3) at (3.5,-0.5) {$\wv(3)\pv(3)$};
% \node (par3) at (3.75,-0.5) {$$};
\node (infoz) at (5.00,-0.5) {$\wv(4) \pv(4)$};
% \node (infoz) at (5.25,-0.5) {$$};

\end{tikzpicture}

==> icassp_rebuttal.tex <==
We begin by expressing our sincere gratitude to the reviewers for their fair, insightful, and constructive feedback. 

As rightfully noted by reviewer 03A3, some constructions of the UBCE (e.g. multi-user PPM) suffer from time asynchrony and, in these situations, equations (1) and (3) are overly simplistic. However, in mMTC and especially URA, concatenated coding techniques are often employed where the inner code protects against channel imperfections (such as asynchrony) and the outer code provides additional error correction or message stitching capabilities (see paragraphs 2-3 of the paper and reference 4). In these situations, the inner code must be (at least partially) decoded before the outer decoder may be run; thus, any asynchrony is ideally corrected before outer decoding begins. In this sense, the UBCE as defined in equations (1) and (3) models the effective channel as seen by the outer code. Admittedly, this concept was not clearly expressed in the introduction. If our paper is accepted, we pledge to clarify the paper with respect to this important point.

Reviewer 16BE wisely recommends that we include more references as well as a qualitative discussion comparing our work to the existing state of the art. We believe this to be a valuable suggestion, especially given the fact that the UBCE is a novel channel model and it is important for readers to understand the similarities and differences between the UBCE and other A/B channel variants. If our paper is accepted, we will provide more context as to how our work fits into the larger landscape of the literature. Furthermore, in connection with feedback from reviewer 03A3, we acknowledge that our paper does not include any performance comparisons with works of other authors. Our initial rationale for this decision was that existing work either does not consider the unsourced part of the UBCE or does not include an erasure process. After careful consideration, we have identified a benchmark from another author that we can adapt and include in the final version of the paper.

As noted by reviewer 03A3, there are errors in the formatting of our references as well as inadequately defined notation. We guarantee that both issues will be rectified in the final version of the paper.

In closing, we would like to thank the reviewers once more for their valuable feedback. We believe that their suggestions will significantly improve the final version of our paper. 





%  
We begin by expressing our sincere gratitude to the reviewers for their fair, insightful, and constructive feedback. 

As rightfully noted by reviewer 03A3, some constructions of the UBCE (e.g. multi-user PPM) suffer from time asynchrony and, in these situations, equations (1) and (3) are overly simplistic. In mMTC, concatenated coding techniques are often employed. In the URA paradigm we envision, the two coding techniques are: (i) inner code that protects against channel imperfections and, (ii) outer code that provides additional error correction or message stitching capabilities (see paragraphs 2-3 of the paper and/or reference 4). In these situations, the inner code must be (at least partially) decoded before the outer decoder may be run; thus, any asynchrony is ideally corrected before outer decoding begins. In this sense, the UBCE as defined in equations (1) and (3) models the effective channel as seen by the outer decoder. Admittedly, this concept was not clearly expressed in the introduction. If our paper is accepted, we pledge to clarify the paper with respect to this important point.

Reviewer 16BE wisely recommends that we include more references as well as a qualitative discussion comparing our work to the existing state of the art. We believe this to be a valuable suggestion, especially given the fact that the UBCE is a novel channel model, and it is important for readers to understand the similarities and differences between the UBCE and other A/B channel variants. If our paper is accepted, we will provide more context as to how our work fits into the larger landscape of the literature. Furthermore, in connection with feedback from reviewer 03A3, we acknowledge that our paper does not include any performance comparisons with works of other authors. Our initial rationale for this decision was that existing work either does not consider the unsourced part of the UBCE or does not include an erasure process. After careful consideration, we have identified a benchmark from another author that we can adapt and include in the final version of the paper.

As noted by reviewer 03A3, there are errors in the formatting of our references as well as inadequately defined notation. We guarantee that both issues will be rectified in the final version of the paper.

In closing, we would like to thank the reviewers once more for their valuable feedback. We believe that their suggestions will significantly improve the final version of our paper.

